Scalar Invariant Networks with Zero Bias

Just like weights, bias terms are the learnable parameters of many popular machine learning models, including neural networks. Biases are thought to enhance the representational power of neural networks, enabling them to solve a variety of tasks in computer vision. However, we argue that biases can be disregarded for some image-related tasks such as image classification, by considering the intrinsic distribution of images in the input space and desired model properties from first principles. Our findings suggest that zero-bias neural networks can perform comparably to biased networks for practical image classification tasks. We demonstrate that zero-bias neural networks possess a valuable property called scalar (multiplication) invariance. This means that the prediction of the network remains unchanged when the contrast of the input image is altered. We extend scalar invariance to more general cases, enabling formal verification of certain convex regions of the input space. Additionally, we prove that zero-bias neural networks are fair in predicting the zero image. Unlike state-of-the-art models that may exhibit bias toward certain labels, zero-bias networks have uniform belief in all labels. We believe dropping bias terms can be considered as a geometric prior in designing neural network architecture for image classification, which shares the spirit of adapting convolutions as the transnational invariance prior. The robustness and fairness advantages of zero-bias neural networks may also indicate a promising path towards trustworthy and ethical AI.

==> 00_abstract.tex <==
\begin{abstract}
% Abstract goes here.

Just like weights, bias terms are the learnable parameters of many popular machine learning models, including neural networks. Biases are believed to effectively increase the representational power of neural networks to solve a wide range of tasks in computer vision. However, we argue that if we consider the intrinsic distribution of images in the input space as well as some desired properties a model should have from the first principles, biases can be completely ignored in addressing many image-related tasks, such as image classification. Our observation indicates that zero-bias neural networks could perform comparably to neural networks with bias at least on practical image classification tasks. In addition, we prove that zero-bias neural networks possess a nice property called scalar (multiplication) invariance, which allows the prediction of neural networks remains the same when altering the contrast of the input image. We then extend scalar invariance to more general cases that allow us to formally verify certain convex regions of the input space. Besides that, we show the fairness of zero-bias neural networks in predicting the zero image. In contrast to the state-of-art models which lean towards certain labels, zero-bias neural networks have a uniform belief in all labels. Based on those merits, we believe dropping bias terms can be considered as a prior in designing neural network architecture for some CV tasks, which shares the spirit of adapting convolutions as the transnational invariance prior.


% \textcolor{red}{
% Our experimental results show that zero-bias models could outperform the state-of-art models by a very large margin (over 60\%) when predicting images under a low illumination condition (multiplying a scalar of 0.01); while achieving the same-level performance as normal models.}



% Our experimental results show that zero-bias models could outperform normally trained models by a very large margin (over 70\%) when predicting images under a low illumination condition (multiplying a scalar of 0.01); while achieving the same-level performance on the test set.





% Our experimental results show that zero-bias SOTA models could classify images correctly 95\% of the time under a low illumination condition (multiplying a scalar of 0.01), outperforming normally trained models by 95\%; while achieving the same-level performance on the test set.









% beat normal SOTA models   by 99\% percent 

% while share comparable performance.
% without hurting performance of models.



% The representation power of NNs without biases. It should be the same as normal NNs when working on image classifications, but not other usual tasks.
% Because the intrinsic distribution of images aligns the patterns of linear regions induced by unbiased NNs. Also, unbiased NNs is much easier to analyze: 1. polarized NNs 2. prediction invariant under rescaling; 3. maybe better robustness properties; 4. study the NAPS of unbiased NNs

% The intrinsic distribution of images in the high-dimensional input space incorporates some directional properties.





\end{abstract}

==> 06_geoinsight.tex <==
\section{Geometric insights}
\label{sec:geo_insights}

\input{linea_reg.tex} 

% \subsection{Geometric insights}
% \label{sec:geo_insights}
Although we have shown that zero-bias neural networks demonstrate some nice properties in terms of robustness, one major concern that emerges along with eliminating bias is the reduction in the representational power of neural networks. Such a reduction may hurt neural networks' performances in certain categories of tasks, yet we argue that image classification tasks seem not to be one of them. Let us consider the intrinsic distribution of images in the high-dimensional input space, illustrated in Figure \ref{fig:Img_dist}. This leads to two key observations:
\begin{itemize}
    \item \textbf{Locality}: The neighborhood with a certain radius of a sample point should belong to the same class.
    \item \textbf{Directionality}: Any points along the direction specified by a sample point should belong to the same class.
\end{itemize}
Since a neural network can be thought of as a piece-wise (linear) function defined over many convex polytopes \cite{LR1,LR2}, we plot linear regions of a simple scalar invariant neural network and a simple normal neural network trained on a simple 2D dataset to study their representational power in Figure \ref{fig:linear_reg}. We consider two easy learning tasks whose input distributions are characterized by \emph{Dir} (directions) 1 and 2. Since locality is implicitly embedded in input distributions of almost every task, including \emph{Dir} 1 and 2 cases (otherwise, generalization is impossible), we mainly discuss the impact of directionality on learning outcomes. First, in the absence of directionality, e.g., in the case of data labeled differently along \emph{Dir} 1, the scalar invariant neural network may not fit data well using only linear function within the corresponding cone, as shown in Figure \ref{fig:linear_regions_nb}. Whereas the normal network could overcome this using a piece-wise linear function across multiple convex regions along \emph{Dir} 1, illustrated in Figure \ref{fig:linear_regions_wb}. \\\\
However, \emph{Dir} 1 is not a serious concern as we observe that the intrinsic distribution of images should incorporate directionality, portrayed by \emph{Dir} 2. We investigate the possible gap in the representational power between the two types of neural networks in the \emph{Dir} 2 case. Given the directionality holds, the scalar invariant neural network could fit the data along that \emph{Dir} 2 using a linear function (within a cone) on par with using piece-wise linear functions by the normal neural networks. This suggests they should deliver comparable performances, and we will provide more experimental evidence to support this claim in Section \ref{sec:exp}.
Following our above discussion, we believe the directionality can be used as a strong geometric prior in image-related tasks, sharing the spirit of adapting transnational invariance prior introduced by CNN. 
It is worth highlighting that a recent line of work~\cite{Liu2017NIPS,Liu2017CVPR,Wen2021SphereFace2,Chen20AVH,https://doi.org/10.48550/arxiv.2206.08704} hold a similar view of the importance of directionality (angle) in image classification and representation learning. Among these work including ours, geometric understanding of image manifold plays an essential role in designing proper methods or injecting correct inductive bias to deep learning research. 

==> _constants.tex <==
\def\cvprPaperID{9991}
\def\confName{CVPR}
\def\confYear{2023}

\def\paperTitle{Scalar Invariant Networks with Zero Bias}

\def\authorBlock{
    Chuqin Geng, Xiaojie Xu, Haolin Ye, Xujie Si
\\
    McGill University \\
    {\tt\small \{chuqin.geng, xiaojie.xu, haolin.ye\}@mail.mcgill.ca, xsi@cs.mcgill.ca}
}




% \author{Chuqin Geng\inst{1,2} \orcidID{0000-0002-3563-1596}\and 
% Haolin Ye\inst{1} \orcidID{0000-0002-7402-617X}\and
% Yixuan Li\inst{1} \orcidID{0000-0001-9349-5476}\and
% Tianyu Han\inst{1} \orcidID{0000-0001-6582-165X}\and
% Brigitte Pientka\inst{1} \orcidID{0000-0002-2549-4276}\and
% Xujie Si\inst{1,2,3} \orcidID{0000-0002-3739-2269} 
% }

% \institute{McGill University
% \and Mila - Quebec Institute
% \and CIFAR AI Research Chair\\
% \email{\{chuqin.geng,haolin.ye,yixuan.li,tianyu.han2\}@mail.mcgill.ca\\
% \{bpientka,xsi\}.cs.mcgill.ca
% }\\


% Compilation vars
\newif\ifreview \newcommand{\review}{\reviewtrue}
\newif\ifarxiv \newcommand{\arxiv}{\arxivtrue}
\newif\ifcamera \newcommand{\cameraready}{\cameratrue}
\newif\ifrebuttal \newcommand{\rebuttal}{\rebuttaltrue}


==> fourier_fig.tex <==
% \begin{figure}[hb!]

%      \centering
%          \includegraphics[width=0.45\textwidth]{figs/fourier/001_cifar100_nfresnet101_bias_energy_plot.png}
%          \label{fig:fourier001_ex1}

%          \centering
%          \includegraphics[width=0.45\textwidth]{figs/fourier/001_cifar100_nfresnet101_nobias_energy_plot.png}
%          \label{fig:fourier001_ex2}
%          \centering
%          \includegraphics[width=0.45\textwidth]{figs/fourier/001_mnist_fcn_bias_energy_plot.png}
%          \label{fig:fourier001_ex3}
%          \centering
%          \includegraphics[width=0.45\textwidth]{figs/fourier/001_mnist_fcn_nobias_energy_plot.png}
%          \label{fig:fourier001_ex4} 
%         \caption{ lr=0.001 }
%         \label{fig:fourier001_example}
% \end{figure}


\begin{figure*}[thb!]
     \centering
    \begin{subfigure}[t]{0.24\textwidth}
         \includegraphics[width=\textwidth]{figs/fourier/0025_fmnist_cnn_bias_energy_plot.pdf}
         \caption{The spectrum of with-bias CNN on Fashion-MNIST.}
         \label{fig:fourier0025_ex3}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}
         \includegraphics[width=\textwidth]{figs/fourier/0025_fmnist_cnn_nobias_energy_plot.pdf}
         \caption{The spectrum of without-bias CNN on Fashion-MNIST.}
         \label{fig:fourier0025_ex4} 
    \end{subfigure}
    \hfill
     \begin{subfigure}[t]{0.24\textwidth}
         \includegraphics[width=\textwidth]{figs/fourier/0025_cifar100_nf_resnet101_bias_energy_plot.pdf}
          \caption{The spectrum of with-bias NF-Resnet on CIFAR100.}
         \label{fig:fourier0025_ex1}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.24\textwidth}

         \includegraphics[width=\textwidth]{figs/fourier/0025_cifar100_nf_resnet101_nobias_energy_plot.pdf}
         \caption{The spectrum of without-bias NF-Resnet on CIFAR100.}
         \label{fig:fourier0025_ex2}
    \end{subfigure}
        \caption{The energy ratio of different frequency components of neural networks during training are portrayed by contour lines. The red and orange curves indicate the errors on the perturbed set (10\% label noise) and the test set, respectively. The differences between the spectrum and errors of zero-bias networks and normal networks are imperceptible, suggesting they have almost identical expressive
capabilities.}
        \label{fig:Fourier_curve}
\end{figure*}

==> learning_curves.tex <==
\begin{figure*}[hbt!]
     \centering
     \begin{subfigure}[t]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/learning_curve/mnist_fcn_accuracy.pdf}
         \caption{Learning curves of FCNs with and without bias on MNIST.}
         \label{fig:ResNet}
     \end{subfigure}
     \hfill
     \begin{subfigure}[t]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/learning_curve/fashionmnist_cnn_accuracy.pdf}
         \caption{Learning curves of CNNs with and without bias on Fashion-MNIST.}
         \label{fig:Inception}
     \end{subfigure}
     \hfill
      \begin{subfigure}[t]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/learning_curve/imagenette_nf_resnet101_accuracy_smltrain_orgtest.pdf}
         \caption{Learning curves of ResNet34 with and without bias on Imagenette.}
         \label{fig:Imagenette}
      \end{subfigure}
     \hfill
    \begin{subfigure}[t]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figs/learning_curve/CIFAR100_nfnet_true.pdf}
         \caption{Learning curves of ResNet101 with and without bias on CIFAR-100.}
         \label{fig:CIFAR10}
     \end{subfigure}
        \caption{Learning curves of normally trained neural networks\textcolor{red}{,} and their scalar invariant
counterparts are almost identical, which supports our argument that removing bias doesn't impact the expressive capability of models on image classification tasks. 
}
        \label{fig:Learning_curve}
\end{figure*}

==> robustness_eval.tex <==
\begin{figure}[hb!]
\centering
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/affect_of_L_infinity_noise_+25.pdf}
        \caption{Adversarial attacks with different number of perturbed pixels to CNN trained on MNIST.}
         \label{fig:Adv_robust_1}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[t]{0.25\textwidth}
        % \centering
         \includegraphics[width=\textwidth]{figs/robustness evaluation/cifar10_nf_resnet18_+0-25.pdf}
         \caption{Adversarial attacks with different number of perturbed pixels to ResNet trained on CIFAR.}
         \label{fig:Adv_robust_2}
    \end{subfigure}
    \caption{Zero-bias networks are more robust against adversarial attacks than with-bias networks; the gap could be explained by the robustness guarantees we proposed. }
    \label{fig:Adversarial_robust_plot}
\end{figure}





         % \includegraphics[width=0.23\textwidth]{figs/robustness evaluation/affect_of_L_infinity_noise_+25.pdf}
         % \label{fig:Adv_robust_2}


% \begin{figure}[t]
%      \begin{subfigure}[t]{0.225\textwidth}
%          \centering         \includegraphics[width=\textwidth]{figs/cvvp1.pdf}
%          \caption{Linear activation regions of a simple scalar invariant neural network are \textit{cones}.} 
%          \label{fig:linear_regions_nb}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[t]{0.225\textwidth}
%          \centering         \includegraphics[width=\textwidth]{figs/cvvp2.pdf}
%          \caption{Linear activation regions of a simple neural network are \textit{polytopes}.}
%          \label{fig:linear_regions_wb}
%          \hfill
%      \end{subfigure}
%         \caption{Scalar invariant neural networks perform poorly along \emph{Dir} 1 (only locality holds) compared to normal neural networks. They perform comparably along \emph{Dir} 2 (both locality and directionality hold).}
        
%         \label{fig:linear_reg}
          
% \end{figure}
\begin{figure}[hb!]
\centering
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_fcn/mnist_fcn_+0-1.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_fcn_0.1}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_fcn/mnist_fcn_+0-15.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_fcn_0.15}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_fcn/mnist_fcn_+0-2.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_fcn_0.2}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_fcn/mnist_fcn_+0-25.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_fcn_0.25}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_fcn/mnist_fcn_+0-3.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_fcn_0.3}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_fcn/mnist_fcn_+0-4.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_fcn_0.4}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_fcn/mnist_fcn_+0-5.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_fcn_0.5}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_fcn/mnist_fcn_+0-6.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_fcn_0.6}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_fcn/mnist_fcn_+0-7.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_fcn_0.7}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_fcn/mnist_fcn_+0-8.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_fcn_0.8}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_fcn/mnist_fcn_+0-9.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_fcn_0.9}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_fcn/mnist_fcn_+1-0.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_fcn_1.0}
     \end{subfigure}
    \caption{MNIST x FCN}
    \label{fig:Adv_robust_mnist_fcn}
\end{figure}



% ===============================================================================================

\begin{figure}[hb!]
\centering
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_cnn/mnist_cnn_+0-1.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_cnn_0.1}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_cnn/mnist_cnn_+0-15.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_cnn_0.15}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_cnn/mnist_cnn_+0-2.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_cnn_0.2}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_cnn/mnist_cnn_+0-25.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_cnn_0.25}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_cnn/mnist_cnn_+0-3.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_cnn_0.3}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_cnn/mnist_cnn_+0-4.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_cnn_0.4}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_cnn/mnist_cnn_+0-5.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_cnn_0.5}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_cnn/mnist_cnn_+0-6.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_cnn_0.6}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_cnn/mnist_cnn_+0-7.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_cnn_0.7}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_cnn/mnist_cnn_+0-8.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_cnn_0.8}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_cnn/mnist_cnn_+0-9.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_cnn_0.9}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/mnist_cnn/mnist_cnn_+1-0.pdf}
        \caption{}
         \label{fig:Adv_robust_mnist_cnn_1.0}
     \end{subfigure}
    \caption{MNIST x CNN}
    \label{fig:Adv_robust_mnist_cnn}
\end{figure}

% ===============================================================================================

\begin{figure}[hb!]
\centering
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/fmnist_cnn/fmnist_cnn_+0-1.pdf}
        \caption{}
         \label{fig:Adv_robust_fmnist_cnn_0.1}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/fmnist_cnn/fmnist_cnn_+0-15.pdf}
        \caption{}
         \label{fig:Adv_robust_fmnist_cnn_0.15}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/fmnist_cnn/fmnist_cnn_+0-2.pdf}
        \caption{}
         \label{fig:Adv_robust_fmnist_cnn_0.2}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/fmnist_cnn/fmnist_cnn_+0-25.pdf}
        \caption{}
         \label{fig:Adv_robust_fmnist_cnn_0.25}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/fmnist_cnn/fmnist_cnn_+0-3.pdf}
        \caption{}
         \label{fig:Adv_robust_fmnist_cnn_0.3}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/fmnist_cnn/fmnist_cnn_+0-4.pdf}
        \caption{}
         \label{fig:Adv_robust_fmnist_cnn_0.4}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/fmnist_cnn/fmnist_cnn_+0-5.pdf}
        \caption{}
         \label{fig:Adv_robust_fmnist_cnn_0.5}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/fmnist_cnn/fmnist_cnn_+0-6.pdf}
        \caption{}
         \label{fig:Adv_robust_fmnist_cnn_0.6}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/fmnist_cnn/fmnist_cnn_+0-7.pdf}
        \caption{}
         \label{fig:Adv_robust_fmnist_cnn_0.7}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/fmnist_cnn/fmnist_cnn_+0-8.pdf}
        \caption{}
         \label{fig:Adv_robust_fmnist_cnn_0.8}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/fmnist_cnn/fmnist_cnn_+0-9.pdf}
        \caption{}
         \label{fig:Adv_robust_fmnist_cnn_0.9}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/fmnist_cnn/fmnist_cnn_+1-0.pdf}
        \caption{}
         \label{fig:Adv_robust_fmnist_cnn_1.0}
     \end{subfigure}
    \caption{FMNIST x CNN}
    \label{fig:Adv_robust_fmnist_cnn}
\end{figure}


% ===============================================================================================

\begin{figure}[hb!]
\centering
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/cifar10_nf_resnet18/cifar10_nf_resnet18_+0-1.pdf}
        \caption{}
         \label{fig:Adv_robust_cifar10_nf_resnet18_0.1}
     \end{subfigure}
     % \hfill
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/cifar10_nf_resnet18/cifar10_nf_resnet18_+0-15.pdf}
        \caption{}
         \label{fig:Adv_robust_cifar10_nf_resnet18_0.15}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/cifar10_nf_resnet18/cifar10_nf_resnet18_+0-2.pdf}
        \caption{}
         \label{fig:Adv_robust_cifar10_nf_resnet18_0.2}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/cifar10_nf_resnet18/cifar10_nf_resnet18_+0-25.pdf}
        \caption{}
         \label{fig:Adv_robust_cifar10_nf_resnet18_0.25}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/cifar10_nf_resnet18/cifar10_nf_resnet18_+0-3.pdf}
        \caption{}
         \label{fig:Adv_robust_cifar10_nf_resnet18_0.3}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/cifar10_nf_resnet18/cifar10_nf_resnet18_+0-4.pdf}
        \caption{}
         \label{fig:Adv_robust_cifar10_nf_resnet18_0.4}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/cifar10_nf_resnet18/cifar10_nf_resnet18_+0-5.pdf}
        \caption{}
         \label{fig:Adv_robust_cifar10_nf_resnet18_0.5}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/cifar10_nf_resnet18/cifar10_nf_resnet18_+0-6.pdf}
        \caption{}
         \label{fig:Adv_robust_cifar10_nf_resnet18_0.6}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/cifar10_nf_resnet18/cifar10_nf_resnet18_+0-7.pdf}
        \caption{}
         \label{fig:Adv_robust_cifar10_nf_resnet18_0.7}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/cifar10_nf_resnet18/cifar10_nf_resnet18_+0-8.pdf}
        \caption{}
         \label{fig:Adv_robust_cifar10_nf_resnet18_0.8}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/cifar10_nf_resnet18/cifar10_nf_resnet18_+0-9.pdf}
        \caption{}
         \label{fig:Adv_robust_cifar10_nf_resnet18_0.9}
     \end{subfigure}
     \begin{subfigure}[t]{0.25\textwidth}
         % \centering                  
         \includegraphics[width=\textwidth]{figs/robustness evaluation/cifar10_nf_resnet18/cifar10_nf_resnet18_+1-0.pdf}
        \caption{}
         \label{fig:Adv_robust_cifar10_nf_resnet18_1.0}
     \end{subfigure}
    \caption{CIFAR10 x NF18}
    \label{fig:Adv_robust_cifar10_nf_resnet18}
\end{figure}

==> tables/backup_table.tex <==
% \begin{table*}[ht]
% \centering
% % \resizebox{\columnwidth}{!}{%
% \resizebox{1.9\columnwidth}{!}{%
% \begin{tabular}{ |c| c |c c c c c c c c c c c |}
% \hline
% \multicolumn{2}{|c|}{}&\multicolumn{11}{c|}{Scalar}\\
% \cline{3-13}
% \multicolumn{2}{|c|}{}&1&0.25&0.15&0.125&0.1&0.075&0.05&0.025&0.01&0.001&0.0001\\ 

% \cline{3-13}
% \hline
% MNIST&w/ bias&88.12&87.07&84.46&82.57&79.52&74.76&65.82&42.84&16.34&10.28&10.28\\
% FCN&w/o bias&88.27&88.27&88.26&88.27&88.27&88.26&88.27&88.27&88.27&88.27&88.27\\
% \hline
% % Fashion-MNIST&w/ bias&98.39&95.89&84.83&75.73&58.62&38.66&25.58&10.57&8.92&8.92&8.92\\
% % CNN&w/o bias&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31\\
% % \hline
% Fashion-MNIST&w/ bias&89.10&67.10&40.12&32.52&24.16&17.91&12.46&10.12&10.00&10.00&10.00\\
% CNN&w/o bias&89.02&89.02&89.02&89.02&89.02&89.02&89.02&89.02&89.02&89.02&89.02\\
% \hline
% CIFAR-100&w/ bias&80.80&81.42&81.04&80.21&78.86&75.70&66.97&44.28&18.27&10.00&10.00\\
% NF\_ResNet&w/o bias&80.34&80.34&80.32&80.34&80.33&80.32&80.33&80.33&80.33&80.32&80.34\\
% \hline
% CIFAR-100&w/ bias&81.11&43.35&15.94&12.13&10.53&10.06&10.00&10.00&10.00&10.00&10.00\\
% Fixup\_ResNet50&w/o bias&81.95&81.95&81.95&81.95&81.95&81.95&81.95&81.95&81.95&81.95&81.96\\
% \hline
% Imagenette&w/ bias&74.98&19.64&10.68&10.04&9.91&9.94&9.91&9.94&9.94&9.94&9.94\\
% Fixup\_ResNet32&w/o bias&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13\\
% \hline
% \end{tabular}
% }

% % }
% \caption{Normal neural networks are generally not robust against scalar multiplication (with the input image), 
% whereas their scalar invariant counterparts achieve absolute invariance
% as we expected.
% }
% \vspace{-0.05in}
% \label{tab:scalar_inv_tab}
% \end{table*}




\begin{table*}[ht]
\centering
% \resizebox{\columnwidth}{!}{%
\resizebox{1.9\columnwidth}{!}{%
\begin{tabular}{ c| c |c c c c c c c c c c c }
\hline
\multicolumn{2}{c|}{}&\multicolumn{11}{c}{Scalar}\\
\cline{3-13}
\multicolumn{2}{c|}{}&1&0.25&0.15&0.125&0.1&0.075&0.05&0.025&0.01&0.001&0.0001\\ 

\cline{3-13}
\hline
MNIST&w/ bias&88.12&87.07&84.46&82.57&79.52&74.76&65.82&42.84&16.34&10.28&10.28\\
FCN&w/o bias&88.27&88.27&88.26&88.27&88.27&88.26&88.27&88.27&88.27&88.27&88.27\\
\hline
% Fashion-MNIST&w/ bias&98.39&95.89&84.83&75.73&58.62&38.66&25.58&10.57&8.92&8.92&8.92\\
% CNN&w/o bias&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31\\
% \hline
Fashion-MNIST&w/ bias&89.10&67.10&40.12&32.52&24.16&17.91&12.46&10.12&10.00&10.00&10.00\\
CNN&w/o bias&89.02&89.02&89.02&89.02&89.02&89.02&89.02&89.02&89.02&89.02&89.02\\
\hline
Imagenette&w/ bias&64.87&19.31&11.80&10.83&10.32&10.19&10.17&10.17&10.17&10.17&10.17\\
Fixup\_ResNet32&w/o bias&59.62&59.62&59.62&59.62&59.62&59.62&59.62&59.62&59.62&59.62&59.62\\
\hline
Imagenette&w/ bias&75.77&72.59&72.19&70.52&65.52&60.36&54.65&33.10&20.20&9.94&9.94\\
NF\_ResNet34&w/o bias&78.45&78.45&78.45&78.45&78.45&78.45&78.45&78.45&78.45&78.45&78.45\\
\hline
\hline
CIFAR-100&w/ bias&63.14&25.05&12.85&9.93&7.42&4.6&2.32&1.16&1.0&1.0&1.0\\
Fixup\_ResNet110&w/o bias&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75\\
\hline
CIFAR-100&w/ bias&61.44&56.21&44.77&39.10&31.00&20.68&9.56&2.79&1.03&1.00&1.00\\\
NF\_ResNet101&w/o bias&62.51&62.51&62.51&62.51&62.51&62.51&62.51&62.51&62.51&62.51&62.51\\
\hline
% CIFAR-100&w/ bias&72.22&71.85&70.34&69.56&67.73&64.37&56.08&30.68&4.74&1.09&1.00\\
% NF\_ResNet101&w/o bias&72.51&72.51&72.51&72.51&72.51&72.51&72.51&72.51&72.51&72.51&72.51\\
% \hline
CIFAR-100, EfficientNet \cite{EfficientNet}&w/ bias&81.94&62.44&40.42&31.81&22.68&13.22&5.39&1.25&1.00&1.00&1.00\\
\hline
CIFAR-100, ViT \cite{ViT}&w/ bias&91.48&81.58&66.11&58.55&47.98&34.11&18.49&4.54&1.08&1.00&1.00\\
\hline
% imagenette, Fixup\_resnet32&w/ bias&64.87&19.31&11.80&10.83&10.32&10.19&10.17&10.17&10.17&10.17&10.17\\
% \hline
\end{tabular}
}

% }
\caption{Normal neural networks are generally not robust against scalar multiplication (with the input image), 
whereas their scalar invariant counterparts achieve absolute invariance
as we expected.
}
\vspace{-0.05in}
\label{tab:scalar_inv_tab}
\end{table*}



% CIFAR-100&w/ bias&0.5872&0.5842&0.5719&0.5655&0.551&0.5234&0.456&0.2495&0.0474&0.0109&0.01\\
% NF\_ResNet101&w/o bias&0.5928&0.5928&0.5928&0.5928&0.5928&0.5928&0.5928&0.5928&0.5928&0.5928&0.5928\\

% CIFAR-100&w/ bias&74.98&19.64&10.68&10.04&9.91&9.94&9.91&9.94&9.94&9.94&9.94\\
% NF\_ResNet101&w/o bias&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13\\

% CIFAR-100&w/ bias&63.14&25.05&12.85&9.93&7.42&4.6&2.32&1.16&1.0&1.0&1.0\\
% Fixup\_ResNet110&w/o bias&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75\\
% \hline




% scalar for compare 1
% 0.6354
% scalar for compare 0.25
% 0.2438
% scalar for compare 0.15
% 0.122
% scalar for compare 0.125
% 0.0964
% scalar for compare 0.1
% 0.0738
% scalar for compare 0.075
% 0.0483
% scalar for compare 0.05
% 0.0231
% scalar for compare 0.025
% 0.0104
% scalar for compare 0.01
% 0.01
% scalar for compare 0.001
% 0.01
% scalar for compare 0.0001
% 0.01






% CIFAR-100&w/ bias&69.14&26.05&13.85&9.93&7.42&4.6&2.32&1.16&1&1&1\\
% Fixup\_ResNet110&w/o bias&69.74&25.38&12.2&9.64&7.38&4.83&2.31&1.04&1.0&1.0&1.0\\
% \hline

==> tables/model_acc_compare.tex <==
% \begin{table*}[ht]
% \centering
% % \resizebox{\columnwidth}{!}{%
% \resizebox{1.9\columnwidth}{!}{%
% \begin{tabular}{ |c| c |c c c c c c c c c c c |}
% \hline
% \multicolumn{2}{|c|}{}&\multicolumn{11}{c|}{Scalar}\\
% \cline{3-13}
% \multicolumn{2}{|c|}{}&1&0.25&0.15&0.125&0.1&0.075&0.05&0.025&0.01&0.001&0.0001\\ 

% \cline{3-13}
% \hline
% MNIST&w/ bias&88.12&87.07&84.46&82.57&79.52&74.76&65.82&42.84&16.34&10.28&10.28\\
% FCN&w/o bias&88.27&88.27&88.26&88.27&88.27&88.26&88.27&88.27&88.27&88.27&88.27\\
% \hline
% % Fashion-MNIST&w/ bias&98.39&95.89&84.83&75.73&58.62&38.66&25.58&10.57&8.92&8.92&8.92\\
% % CNN&w/o bias&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31\\
% % \hline
% Fashion-MNIST&w/ bias&89.10&67.10&40.12&32.52&24.16&17.91&12.46&10.12&10.00&10.00&10.00\\
% CNN&w/o bias&89.02&89.02&89.02&89.02&89.02&89.02&89.02&89.02&89.02&89.02&89.02\\
% \hline
% CIFAR-100&w/ bias&80.80&81.42&81.04&80.21&78.86&75.70&66.97&44.28&18.27&10.00&10.00\\
% NF\_ResNet&w/o bias&80.34&80.34&80.32&80.34&80.33&80.32&80.33&80.33&80.33&80.32&80.34\\
% \hline
% CIFAR-100&w/ bias&81.11&43.35&15.94&12.13&10.53&10.06&10.00&10.00&10.00&10.00&10.00\\
% Fixup\_ResNet50&w/o bias&81.95&81.95&81.95&81.95&81.95&81.95&81.95&81.95&81.95&81.95&81.96\\
% \hline
% Imagenette&w/ bias&74.98&19.64&10.68&10.04&9.91&9.94&9.91&9.94&9.94&9.94&9.94\\
% Fixup\_ResNet32&w/o bias&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13\\
% \hline
% \end{tabular}
% }

% % }
% \caption{Normal neural networks are generally not robust against scalar multiplication (with the input image), 
% whereas their scalar invariant counterparts achieve absolute invariance
% as we expected.
% }
% \vspace{-0.05in}
% \label{tab:scalar_inv_tab}
% \end{table*}




\begin{table*}[ht]
\centering
% \resizebox{\columnwidth}{!}{%
\resizebox{1.9\columnwidth}{!}{%
\begin{tabular}{ c|c| c |c c c c c c c c c c c }
\hline
\multicolumn{3}{c|}{}&\multicolumn{11}{c}{Scalar}\\
\cline{4-14}
\multicolumn{3}{c|}{}&1&0.25&0.15&0.125&0.1&0.075&0.05&0.025&0.01&0.001&0.0001\\ 

\cline{4-14}
\hline
\multirow{2}{*}{MNIST}&\multirow{2}{*}{FCN}&w/ bias&88.12&87.07&84.46&82.57&79.52&74.76&65.82&42.84&16.34&10.28&10.28\\
&&w/o bias&\textbf{88.27}&\textbf{88.27}&\textbf{88.26}&\textbf{88.27}&\textbf{88.27}&\textbf{88.26}&\textbf{88.27}&\textbf{88.27}&\textbf{88.27}&\textbf{88.27}&\textbf{88.27}\\
\hline
% Fashion-MNIST&w/ bias&98.39&95.89&84.83&75.73&58.62&38.66&25.58&10.57&8.92&8.92&8.92\\
% CNN&w/o bias&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31&98.31\\
% \hline
\multirow{2}{*}{Fashion-MNIST}&\multirow{2}{*}{CNN}&w/ bias&\textbf{89.10}&67.10&40.12&32.52&24.16&17.91&12.46&10.12&10.00&10.00&10.00\\
&&w/o bias&89.02&\textbf{89.02}&\textbf{89.02}&\textbf{89.02}&\textbf{89.02}&\textbf{89.02}&\textbf{89.02}&\textbf{89.02}&\textbf{89.02}&\textbf{89.02}&\textbf{89.02}\\
\hline
\multirow{4}{*}{Imagenette\cite{Howard_Imagenette_2019}}&\multirow{2}{*}{Fixup\_ResNet32}&w/ bias&64.87&19.31&11.80&10.83&10.32&10.19&10.17&10.17&10.17&10.17&10.17\\
&&w/o bias&59.62&59.62&59.62&59.62&59.62&59.62&59.62&59.62&59.62&59.62&59.62\\
\cline{2-14}
&\multirow{2}{*}{NF\_ResNet34}&w/ bias&75.77&72.59&72.19&70.52&65.52&60.36&54.65&33.10&20.20&9.94&9.94\\
&&w/o bias&\textbf{78.45}&\textbf{78.45}&\textbf{78.45}&\textbf{78.45}&\textbf{78.45}&\textbf{78.45}&\textbf{78.45}&\textbf{78.45}&\textbf{78.45}&\textbf{78.45}&\textbf{78.45}\\
\hline
\hline
\multirow{6}{*}{CIFAR-100}&\multirow{2}{*}{Fixup\_ResNet110}&w/ bias&63.14&25.05&12.85&9.93&7.42&4.6&2.32&1.16&1.0&1.0&1.0\\
&&w/o bias&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75\\
\cline{2-14}
&\multirow{2}{*}{NF\_ResNet101} &w/ bias&61.44&56.21&44.77&39.10&31.00&20.68&9.56&2.79&1.03&1.00&1.00\\\
&&w/o bias&62.51&62.51&62.51&\textbf{62.51}&\textbf{62.51}&\textbf{62.51}&\textbf{62.51}&\textbf{62.51}&\textbf{62.51}&\textbf{62.51}&\textbf{62.51}\\
\cline{2-14}
% CIFAR-100&w/ bias&72.22&71.85&70.34&69.56&67.73&64.37&56.08&30.68&4.74&1.09&1.00\\
% NF\_ResNet101&w/o bias&72.51&72.51&72.51&72.51&72.51&72.51&72.51&72.51&72.51&72.51&72.51\\
% \hline
& EfficientNet \cite{EfficientNet}&w/ bias&81.94&62.44&40.42&31.81&22.68&13.22&5.39&1.25&1.00&1.00&1.00\\
\cline{2-14}
& ViT \cite{ViT}&w/ bias&\textbf{91.48}&\textbf{81.58}&\textbf{66.11}&58.55&47.98&34.11&18.49&4.54&1.08&1.00&1.00\\
\hline
% imagenette, Fixup\_resnet32&w/ bias&64.87&19.31&11.80&10.83&10.32&10.19&10.17&10.17&10.17&10.17&10.17\\
% \hline
\end{tabular}
}

% }
\caption{Normal neural networks are generally not robust against scalar multiplication (with the input image), 
whereas their scalar invariant counterparts achieve absolute invariance
as we expected.
}
\vspace{-0.05in}
\label{tab:scalar_inv_tab}
\end{table*}



% CIFAR-100&w/ bias&0.5872&0.5842&0.5719&0.5655&0.551&0.5234&0.456&0.2495&0.0474&0.0109&0.01\\
% NF\_ResNet101&w/o bias&0.5928&0.5928&0.5928&0.5928&0.5928&0.5928&0.5928&0.5928&0.5928&0.5928&0.5928\\

% CIFAR-100&w/ bias&74.98&19.64&10.68&10.04&9.91&9.94&9.91&9.94&9.94&9.94&9.94\\
% NF\_ResNet101&w/o bias&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13&68.13\\

% CIFAR-100&w/ bias&63.14&25.05&12.85&9.93&7.42&4.6&2.32&1.16&1.0&1.0&1.0\\
% Fixup\_ResNet110&w/o bias&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75&53.75\\
% \hline




% scalar for compare 1
% 0.6354
% scalar for compare 0.25
% 0.2438
% scalar for compare 0.15
% 0.122
% scalar for compare 0.125
% 0.0964
% scalar for compare 0.1
% 0.0738
% scalar for compare 0.075
% 0.0483
% scalar for compare 0.05
% 0.0231
% scalar for compare 0.025
% 0.0104
% scalar for compare 0.01
% 0.01
% scalar for compare 0.001
% 0.01
% scalar for compare 0.0001
% 0.01






% CIFAR-100&w/ bias&69.14&26.05&13.85&9.93&7.42&4.6&2.32&1.16&1&1&1\\
% Fixup\_ResNet110&w/o bias&69.74&25.38&12.2&9.64&7.38&4.83&2.31&1.04&1.0&1.0&1.0\\
% \hline

==> vis_inv.tex <==
\begin{figure*}[hbt!]
     \centering
     \begin{subfigure}[t]{\textwidth}
         \centering
         \includegraphics[width=0.95\textwidth]{figs/gradient_pictures/imagenette_idx1047_gt3_with_text.pdf}
         \label{fig:vis_inv_1}
     \end{subfigure}
     \vfill
    \begin{subfigure}[t]{\textwidth}
         \centering
         \includegraphics[width=0.95\textwidth]{figs/gradient_pictures/imagenette_idx3130_gt8_with_text.pdf}
         \label{fig:vis_inv_4}
     \end{subfigure}
     \vfill
      \begin{subfigure}[t]{\textwidth}
         \centering
         \includegraphics[width=0.95\textwidth]{figs/gradient_pictures/imagenette_idx3752_gt5_with_text.pdf}
         \label{fig:vis_inv_5}
      \end{subfigure}
        \caption{ Prediction of normally trained neural networks changes constantly as the scalar decreases, whereas that of zero-bias networks remains unchanged.}
        \label{fig:vis_inv_all}
\end{figure*}



     % \vfill
     % \begin{subfigure}[t]{\textwidth}
     %     \centering
     %     \includegraphics[width=0.95\textwidth]{figs/gradient_pictures/imagenette_idx2701_gt1_with_text.pdf}
     %     \label{fig:vis_inv_2}
     % \end{subfigure}


% \begin{figure*}[hbt!]
%      \centering
%      \begin{subfigure}[t]{\textwidth}
%          \centering
%          \includegraphics[width=0.95\textwidth]{figs/gradient_pictures/imagenette_idx1047_gt3_with_text.pdf}
%          \label{fig:vis_inv_1}
%      \end{subfigure}
%      \vfill
%      \begin{subfigure}[t]{\textwidth}
%          \centering
%          \includegraphics[width=0.95\textwidth]{figs/gradient_pictures/imagenette_idx2701_gt1_with_text.pdf}
%          \label{fig:vis_inv_2}
%      \end{subfigure}
%      \vfill
%     \begin{subfigure}[t]{\textwidth}
%          \centering
%          \includegraphics[width=0.95\textwidth]{figs/gradient_pictures/imagenette_idx3360_gt6_with_text.pdf}
%          \label{fig:vis_inv_3}
%      \end{subfigure}
%      \vfill
%     \begin{subfigure}[t]{\textwidth}
%          \centering
%          \includegraphics[width=0.95\textwidth]{figs/gradient_pictures/imagenette_idx3130_gt8_with_text.pdf}
%          \label{fig:vis_inv_4}
%      \end{subfigure}
%      \vfill
%       \begin{subfigure}[t]{\textwidth}
%          \centering
%          \includegraphics[width=0.95\textwidth]{figs/gradient_pictures/imagenette_idx3752_gt5_with_text.pdf}
%          \label{fig:vis_inv_5}
%       \end{subfigure}
%         \caption{\textit{W/ bias} and \textit{w/o bias} stand for the prediction of normal and scalar invariant models respectively. Prediction of normally trained neural networks changes constantly as the scalar decreases, whereas that of scalar invariant networks remains unchanged. Despite the probability of the corresponding class diminishing. models inherit scalar invariance from removing bias.
% }
%         \label{fig:vis_inv_all}
% \end{figure*}


    % \begin{subfigure}[t]{\textwidth}
    %      \centering
    %      \includegraphics[width=0.9\textwidth]{figs/gradient_pictures/imagenette_idx3130_gt8_with_text.pdf}
    %      \label{fig:vis_inv_4}
    %  \end{subfigure}
